Multi-Stream Cellular Test-Time Adaptation of Real-Time Models Evolving in Dynamic Environments

In the era of the Internet of Things (IoT), objects connect through a dynamic network, empowered by technologies like 5G, enabling real-time data sharing. However, smart objects, notably autonomous vehicles, face challenges in critical local computations due to limited resources. Lightweight AI models offer a solution but struggle with diverse data distributions. To address this limitation, we propose a novel Multi-Stream Cellular Test-Time Adaptation (MSC-TTA) setup where models adapt on the fly to a dynamic environment divided into cells. Then, we propose a real-time adaptive student-teacher method that leverages the multiple streams available in each cell to quickly adapt to changing data distributions. We validate our methodology in the context of autonomous vehicles navigating across cells defined based on location and weather conditions. To facilitate future benchmarking, we release a new multi-stream large-scale synthetic semantic segmentation dataset, called DADE, and show that our multi-stream approach outperforms a single-stream baseline. We believe that our work will open research opportunities in the IoT and 5G eras, offering solutions for real-time model adaptation.

==> tables/Result_mIoU_dynamic.tex <==

\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|}
        \multicolumn{3}{c}{} &  \multicolumn{2}{|c}{\textbf{mIoU imminent}} &  \multicolumn{2}{|c|}{\textbf{mIoU future}}\\ \hline
        \textbf{Pretraining}     & \textbf{Scenario}           & \textbf{Adapt}                 & 5 hours & Last hour & 5 hours & Last hour\\ \hline
        \multirow{6}{*}{Scratch}         & Baseline           & \checkmark                    & .204 & .197 & .167 & .167\\
                 & General            & \checkmark                    & \uline{.278} & \uline{.352} & \uline{.249} & \uline{.323}\\
                 & Spatial            & \checkmark                    & \textbf{.307} & \textbf{.397} & \textbf{.269} & \textbf{.358}\\
                 & Weather            & \checkmark                    & .226 & .295 & .199 & .279\\
                 & Daylight           & \checkmark                    & .245 & .279 & .176 & .259\\
                 & Specific           & \checkmark                    & .22  & .204 & .203 & .187\\ \hline
        \multirow{7}{*}{General}         & Baseline           & \checkmark                    & .581 & .546 & .502 & .502\\
                 & General            & \checkmark                    & \uline{.644} & .595 & \uline{.613} & .565\\
                 & Spatial            & \checkmark                    & \textbf{.654} & \textbf{.622} & .606 & \textbf{.589}\\
                 & Weather            & \checkmark                    & .641 & .586 & .611 & .562\\
                 & Daylight           & \checkmark                    & .636 & \uline{.603} & .572 & \uline{.585}\\
                 & Specific           & \checkmark                    & .632 & .602 & .596 & .559\\ 
                 & General            & -                             & .618 & .581 & \textbf{.618} & .581\\ \hline
        \multirow{8}{*}{Cell}            & Spatial            & \checkmark                    & \uline{.6} & \textbf{.575} & .551 & .541\\
                    & Weather            & \checkmark                    & .577 & .523 & .546 & .497\\
                    & Daylight           & \checkmark                    & \textbf{.613} & \uline{.567} & .543 & \textbf{.557}\\
                    & Specific           & \checkmark                    & .435 & .447 & .412 & .421\\
                    & Spatial            & -                             & .557 & .529 & \uline{.557} & .529\\
                    & Weather            & -                             & .535 & .495 & .535 & .495\\
                    & Daylight           & -                             & .594 & .554 & \textbf{.594} & \uline{.554}\\
                    & Specific           & -                             & .41  & .446 & .41  & .446\\

    \end{tabular}}
    \caption{Aggregated performances for dynamic weather. For the same pretraining and each metric, the first score is in \textbf{bold} and the second is \uline{underlined}.}
    \label{tab:agg_dw}
\end{table}

==> tables/Result_mIoU_static.tex <==

\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|}
        \multicolumn{3}{c}{} &  \multicolumn{2}{|c}{\textbf{mIoU imminent}} &  \multicolumn{2}{|c|}{\textbf{mIoU future}}\\ \hline
        \textbf{Pretraining}     & \textbf{Scenario}           & \textbf{Adapt}                 & 5 hours & Last hour & 5 hours & Last hour\\ \hline
        \multirow{3}{*}{Scratch}         & Baseline           & \checkmark                    & .223 & .249 & .208 & .231\\
                 & General            & \checkmark                    & \uline{.338} & \uline{.483} & \uline{.316} & \uline{.461}\\
                 & Spatial            & \checkmark                    & \textbf{.353} & \textbf{.513} & \textbf{.328} & \textbf{.485}\\ \hline
        \multirow{4}{*}{General}         & Baseline           & \checkmark                    & .435 & .442 & .415 & .446\\
                 & General            & \checkmark                    & \textbf{.702} & \uline{.696} & \textbf{.673} & \uline{.692}\\           
                 & Spatial            & \checkmark                    & \uline{.700} & \textbf{.701} & \uline{.660} & \textbf{.701}\\
                 & General            & -                             & .650 & .658 & .650 & .658\\\hline
        \multirow{2}{*}{Cell}            & Spatial            & \checkmark                    & \textbf{.658} & \textbf{.681} & \uline{.597} & \textbf{.682}\\      
                 & Spatial            & -                             & \uline{.634} & \uline{.660} & \textbf{.634} & \uline{.660}\\
        \hline\\
        \hline
        \multirow{3}{*}{Scratch}         & Baseline           & \checkmark                    & .274 & .309 & .244 & .285\\
                 & General            & \checkmark                    & \uline{.340} & \uline{.363} & \uline{.327} & \uline{.373}\\
                 & Spatial            & \checkmark                    & \textbf{.368} & \textbf{.440} & \textbf{.351} & \textbf{.413}\\ \hline
        \multirow{4}{*}{General}         & Baseline           & \checkmark                    & .422 & .442 & .397 & .425\\
                 & General            & \checkmark                    & \textbf{.474} & \textbf{.517} & \uline{.461} & \uline{.501}\\
                 & General            & -                             & .454 & \uline{.450} & .454 & .450\\
                 & Spatial            & \checkmark                    & \uline{.470} & \textbf{.517} & \textbf{.462} & \textbf{.505}\\ \hline
        \multirow{2}{*}{Cell}            & Spatial            & \checkmark                    & \textbf{.552} & \uline{.567} & \uline{.522} & \uline{.556}\\    
                 & Spatial            & -                             & \uline{.544} & \textbf{.572} & \textbf{.544} & \textbf{.572}\\

    \end{tabular}}
    \caption{Aggregated performances for static weather. For the same pretraining and each metric, the first score is in \textbf{bold} and the second is \uline{underlined}.}
    \label{tab:agg_sw}
\end{table}

==> tables/Resume_partition.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c}
                         & \multicolumn{2}{c|}{\textbf{Static Weather}} & \multicolumn{2}{c}{\textbf{Dynamic Weather}} \\ 
\textbf{Scenarios}        & $\agentSize$   & $\environmentSize$ & $\agentSize$   & $\environmentSize$  \\ \hline
Baseline                 & 1              & 1            & 1              & 1             \\ \hline
General                  & 67            & 1            & 199           & 1             \\ \hline
Spatial                  & 67           & 7            & 199           & 7             \\ \hline
Weather                  & -              & -            & 199          & 3             \\ \hline
Daylight                 & -              & -            & 199          & 2             \\ \hline
Weather + Daylight     & -              & -            & 199          & 6             \\ \hline
Spatial + Weather + Daylight                & -              & -            & 199         & 42            \\ \hline
\end{tabular}}
\caption{Summary of the different environment division that we study in our experiments, where $\agentSize$ is the number of agents (in the TTA set) and $\environmentSize$ is the number of cells in which the dynamic environment is divided.}
\label{tab:partition_description}
\end{table}

